Lagrangian Neural Style Transfer for Fluids

Artistically controlling the shape, motion and appearance of fluid simulations pose major challenges in visual effects production. In this paper, we present a neural style transfer approach from images to 3D fluids formulated in a Lagrangian viewpoint. Using particles for style transfer has unique benefits compared to grid-based techniques. Attributes are stored on the particles and hence are trivially transported by the particle motion. This intrinsically ensures temporal consistency of the optimized stylized structure and notably improves the resulting quality. Simultaneously, the expensive, recursive alignment of stylization velocity fields of grid approaches is unnecessary, reducing the computation time to less than an hour and rendering neural flow stylization practical in production settings. Moreover, the Lagrangian representation improves artistic control as it allows for multi-fluid stylization and consistent color transfer from images, and the generality of the method enables stylization of smoke and liquids likewise.

==> LNST arxiv (1)/include.tex <==
% Some useful commands:
\usepackage[normalem]{ulem}
\usepackage{stackengine}
\usepackage{subfigure}
\usepackage{graphicx}
% \usepackage{subcaption}
\usepackage{float}

\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand\red{\color{red}}
\newcommand\green{\color{cyan}}
\newcommand\blue{\color{blue}}
\newcommand\brown{\color{brown}}
\newcommand\orange{\color{purple}}
\newcommand\wrong[1]{{\color{red}#1}}
\newcommand\gray{\color{gray}}


\newcommand{\todo}[1]{}

\newcommand\hide[1]{}
\newcommand\remove[1]{{\red \sout{#1}}}
\newcommand\removeWnote[2]{{\red \sout{#1}} {\textit{\gray(#2)}}}
\newcommand{\replace}[2]{{\red \sout{#1}} {\blue #2}}
\newcommand\add[1]{{#1}}
\newcommand\addWComment[2]{{\blue #1} {\textit{\gray(#2)}}}
\newcommand\review[1]{{\orange #1}}
\newcommand\highlight[1]{{\green #1}}
\newcommand\reviewWComment[2]{{\orange #1} {\textit{\gray(#2)}}}
\newcommand\addComment[1]{\textit{\gray(#1)}}
\newcommand\revise[1]{{\red #1}}

\definecolor{bkcolor}{RGB}{210,10,210}
\definecolor{vcacolor}{RGB}{123,50,210}
\definecolor{barbaracolor}{RGB}{246,150,70}
\newcommand{\bk}[1]{{\color{bkcolor}\textbf{BK:} #1}}
\newcommand{\vca}[1]{{\color{vcacolor}{\textbf{VCA:} #1}}}
\newcommand{\bs}[1]{{\color{barbaracolor}\textbf{BS:} #1}}

\newcommand\ie{i.e.,~}
\newcommand\eg{e.g.,~}
\newcommand\Fig[1]{Figure~\ref{fig:#1}}
\newcommand\Sec[1]{Section~\ref{sec:#1}}
\newcommand\Eq[1]{Equation~(\ref{eq:#1})}
\newcommand\Eqs[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand\Algo[1]{Algorithm~(\ref{algo:#1})}
\newcommand\Tab[1]{Table~(\ref{tab:#1})}

\newcommand\gradU{\nabla \vec{u}}

%Words unification commands: feel free to change ;)
\newcommand\dataset{dataset}
\newcommand\datasets{datasets}
\newcommand\twoD{2D}
\newcommand\threeD{3D}
\newcommand\particleToGrid{particle-to-grid}
\newcommand\gridToParticle{grid-to-particle}
\newcommand\maxSpeedUp{$x36$}

%Are we going for reduced-order methods or reduced-order models?
\newcommand\roms{reduced-order methods}
\newcommand\Roms{Reduced-order methods}
\newcommand\RoMs{Reduced-order Methods}
\newcommand\cnnName{Deep Fluids}

\newcommand{\Vdim}{V_{\textrm{dim}}}
\newcommand{\Gdim}{G_{\textrm{dim}}}
\newcommand{\dmax}{d_{\textrm{max}}}
\newcommand{\Cdim}{c_{\textrm{dim}}}
\newcommand{\Pdim}{p_{\textrm{dim}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\eqdef}{\overset{def}{=}}

\newcommand\tablefont[1]{\small{#1}}
\newcommand\imagefont[1]{\footnotesize{#1}} 

\newcommand{\gridSuper}{\fbox{\small{+}}}
\newcommand{\particleSuper}{\circ}
\newcommand{\grid}[1]{#1^{\setlength{\fboxsep}{0pt}\gridSuper}}
\newcommand{\particle}[1]{#1^{\particleSuper}}

==> LNST arxiv (1)/sec/eulerianTNST.tex <==

\section{Eulerian Transport-Based NST}
\label{sec:Preliminaries}
We briefly review previous Eulerian-based TNST \cite{Kim2019} for completeness and to better compare against our novel Lagrangian approach. Transport-Based Neural Style Transfer (TNST) extends the original NST algorithm to transfer the style of a given image to a flow-based 3D smoke density. As opposed to NST where individual pixels of the target image are optimized, TNST optimizes a velocity field that modifies density values through indirect smoke transport. The velocity field $\hat{\vec{v}}$ that stylizes the input density $d$ is defined by a loss function $\mathcal{L}$ computed from a pre-trained image classification CNN by 
%
\begin{equation}
\hat{\vec{v}} = \argmin_{\vec{v}} \sum_{\theta \in \Theta} \mathcal{L}(\mathcal{R}_\theta(\mathcal{T}(d,\vec{v}))\,, \vec{p}),
\label{eq:tnstSingle}
\end{equation}
%
where $\mathcal{T}$ is a transport function that advects $d$ with $\vec{v}$, generating the stylized density $\hat{d}=\mathcal{T}(d,\hat{\vec{v}})$; $\mathcal{R}$ is a differentiable renderer converting the density field to image-space for a specific view $\theta$ by $I = \mathcal{R}_{\theta}(\hat{d})$, and $\vec{p}$ denotes the set of user-defined parameters used in the stylization process. The velocity field contributions are individually computed per view, resulting in a \threeD~volumetric smoke stylization. While the authors separate the velocity field into its irrotational and incompressible parts which can be optimized independently, we omit this here for simplicity. 


%While the original \add{image $I$} 
The loss function is subdivided into semantic and style losses for additional control over artistic stylization given a rendered density field. Style transfer considers an input image and user-selected activation layers (levels of features), while semantic transfer selects a CNN layer with desirable attributes that will be transferred to the target stylized smoke. Since the smoke is advected towards a target objective, this guarantees that the original smoke shape and semantics is enforced without matching its original content loss, as in traditional NST algorithms \cite{gatys2015neural}. For simplicity, we restrict our discussion to the style loss, which is given by
%
%The loss function of \eq{tnstSingle} is subdivided as weighted summations of content and style losses
%
%\begin{equation}
%\begin{split}
%\mathcal{L}(\hat{I}, \vec{p}) & = \alpha \mathcal{L}_c(I, \vec{p}) + \beta %\mathcal{L}_s(I, \vec{p}),\\
%\end{split}
%\label{eq:lossDecomposition}
%\end{equation}
%
%where the content loss is given by filter response activations
%
%\begin{equation}\label{eq:semanticLoss}
%\mathcal{L}_c(I, \vec{p}_c) = \sum_l^{L} \left [ \frac{1}{H_l W_l C_l} \sum_i^{H_l} \sum_j^{W_l} \sum_k^{C_l} \left(\mathcal{F}^l_{ijk}(I) - \mathcal{M}^l_{ijk}\right)^2 \right ],
%\end{equation}
%
%and the style loss is 
%
\begin{equation}
\mathcal{L}_s(I, \vec{p}_s) = \sum_l^{L} \left [ \frac{1}{4C_l^2 (H_l\times W_l)^2} \sum_{m, n}^{C_l} \left( G^l_{mn}(I) - G^l_{mn}(I_s) \right)^2 \right ],
\label{eq:styleTransferFinal}
\end{equation}
%
where the Gram matrix $G$ computes correlations between different filter responses. The Gram matrix is calculated for a given layer $l$ and two channels $m$ and $n$, by iterating over all pixels of the flattened 1-D \add{feature map} $\mathcal{\hat{F}}^l(I)$ as
%
\begin{equation}
G^l_{mn}(I) = \sum_{i}^{H_l\times W_l} \mathcal{\hat{F}}_{mi}^l(I) \; \mathcal{\hat{F}}_{ni}^l(I).
\end{equation}
%
%\add{where $i$ iterates over all pixels of the flattened 1-D filter $\mathcal{\hat{F}}^l(I)$. }

%The loss function is computed by
Extending the single frame stylization in a time-coherent fashion is expensive and inaccurate when computed in an Eulerian framework.
TNST aligns stylization velocities by recursively advecting them with the simulation velocities for a given window size as shown in \Fig{tnstalign}. The recursive nature renders this computation inefficient time- and memory-wise, especially when large window sizes are employed to enable smooth transitions between consecutive frames. Due to the large memory requirement, this operation often has to be computed on the CPU, which generates additional overhead by the use of expensive data transfer operations. 
%
\begin{figure} [h!]
  \centering
  \includegraphics[width=0.435\textwidth]{fig/method/tnst_align.png}
  \caption{Recursive temporal alignment in TNST. For a window size $w$, $(w^2-1)/4$ recursive temporal alignment steps are performed for each stylization velocity $\hat{\vec{v}}$.
  %\replace{\add{Each color represents a distance from a frame $t$, and arrows represent the advections (dashed line for the recursive one from further frames).}}
  \add{Colors indicate the distance to frame $t$, and arrows refer to advection steps (with recursive steps shown as dashed lines). 
  }
  }
  %\replace{Recursive temporal alignment of a window size $w=9$ in TNST.}{\bk{In TNST, $(w^2-1)/4$ times of recursive temporal alignment are performed for each stylization velocity $\hat{\vec{v}}$ with a window size $w$.}}} %  \addComment{explain what colors mean}
  \label{fig:tnstalign}
\end{figure}
%
%In the time-coherent multi-view stylization \eq{eq:tnstSingle} is rewritten as
%
%\begin{equation}\label{eq:objfinal}
%\hat{\vec{v}} = \argmin_{\vec{v}_t} \sum_{i=t-w}^{t+w} \sum_{\theta \in \Theta} \mathcal{L}(\mathcal{R}_\theta(\mathcal{T}(d_i,\vec{v}^\ast_i))\,, \vec{p}),
%\end{equation}

%\add{Previously, the authors circumvent this memory requirement by performing velocity alignments back on the cpu, which makes the method additionally slow. } \addComment{\vca{Discuss limitations of previous TNST algorithm.}}
%
%


==> LNST arxiv (1)/sec/introduction.tex <==
\section{Introduction}

%\begin{figure*}[t!]
%    \centering
%    \includegraphics[trim=0px 0px 0px 0px, clip, width=0.8\textwidth]{fig/method/pipeline}
%    \caption{\revise{Method overview} \addComment{remove copied images from TNST}}
%    \label{fig:pipeline}
%    \vspace{-5px}
%\end{figure*}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.75\textwidth]{fig/overview/overview}
    \caption{
    %\replace{Overview of our LNST method. Contrary to TNST, particle positions $\particle{\vec{x}}$ and its attributes $\particle{\lambda}$ are given as input. Either $\particle{\vec{x}}$ or $\particle{\lambda}$ are iteratively optimized to stylize given density field, represented by $d^*$ with splatting operation $\mathcal{I}_{p2g}$. To accommodate grid-based representations as input as TNST, we provide an multi-scale particle resampling method (\Algo{densitySample}). The objective and multi-scale stylization scheme are identical to TNST.}
    \add{Overview of our LNST method. We optimize particle positions $\particle{\vec{x}}$ and attributes $\particle{\lambda}$ to stylize a given density field $d^*$. We transfer information from particles to the grid with the splatting operation $\mathcal{I}_{p2g}$, and jointly update loss functions and attributes. 
    The black arrows show the direction of the feed-forward pass to the loss network $L$, and the gray arrows indicate backpropagation for computing gradients.
    For grid-based simulation inputs, we sample and re-simulate particles in a multi-scale manner (\Algo{densitySample}).}
    }
    \label{fig:overview}
    \vspace{-5px}
\end{figure*}
%

%  On the left, three input fields $d, \Phi, \vec{\Psi}$ for the stylization algorithm are shown. $\Phi, \vec{\Psi}$ are iteratively updated during the optimization, while the stylized density output is represented by $d^*$. All fields are firstly downsampled and stylized on their coarser representations, so features can be enhanced through larger regions of the smoke. Cubic upsampling is performed on $d, \Phi, \vec{\Psi}$ and the stylization runs again on a finer resolution; this process repeats until the specified resolution is matched. The right side of the diagram illustrates how our optimization works. The black arrows show the direction of a feed-forward pass from potentials $\Phi, \vec{\Psi}$ to the loss network, and the gray arrows represent the backpropagation path for computing gradients.}

%\replace{ Artistically manipulating fluid simulations is a challenging task. The high non-linearity of the underlying fluid motion equations hinders optimization, and keyframe-matching designed frames through fully-optimized simulations \cite{Treuille2003, McNamara2004, Pan2016} is computationally expensive while offering limited artistic capabilities. Thus, techniques like proportional-derivative controllers \cite{Fattal2004}, guideline shapes \cite{Nielsen2011}, patch-based texture composition \cite{Jamriska2015}, or turbulent synthesis \cite{kim2008,sato2018example} are commonly employed to manipulate fluid simulations.  Recently, Kim et al. \shortcite{Kim2019} extended the traditional Neural Style Transfer (NST) for images \cite{gatys2016} to volumetric 3D smoke data, obtaining \replace{impressive automatically created smoke stylizations from single images.}{stylized smoke structures based on example images.} Their approach \replace{offered unmatched transferring of}{can transfer} complex styles and semantic structures, ranging from simple image patterns to intricate motifs. 
%}

In visual effects production, physics-based simulations are not only used to realistically re-create natural phenomena, but also as a tool to convey stories and trigger emotions. Hence, artistically controlling the shape, motion and the appearance of simulations is essential for providing directability for physics. Specifically to fluids, the major challenge is the non-linearity of the underlying fluid motion equations, which makes optimizations towards a desired target difficult. Keyframe matching either through expensive fully-optimized simulations \cite{Treuille2003, McNamara2004, Pan2016} or simpler distance-based forces \cite{Nielsen2011,Raveendran2012} provide control over the shape of fluids. The fluid motion can be enhanced with turbulence synthesis approaches \cite{kim2008wavelet,sato2018example} or guided by coarse grid simulations \cite{Nielsen2011}, while patch-based texture composition \cite{Gagnon2019, jamrivska2015lazyfluids} enables manipulation over appearance by automatic transfer of input 2D image patterns. %\add{All the aforementioned techniques, however, are limited to their own scope. }

%\addComment{\vca{So for the paragraph above I think that its a cool structure to mention about the 3 aspects that we mentioned about directability for fluids: shape (keyframe or guide-shapes), motion (turbulence or coarse resolutions) and appearance (patch-based texture transfer). The next paragraph limits down our contributions to appearance and motion  only}}

The recently introduced Transport-based Neural Style Transfer (TNST) \cite{Kim2019} takes flow appearance and motion control to a new level: arbitrary styles and semantic structures given by 2D input images are automatically transferred to 3D smoke simulations. The achieved effects range from natural turbulent structures to complex artistic patterns and intricate motifs. The method extends traditional image-based Neural Style Transfer \cite{gatys2016} by reformulating it as a transport-based optimization. Thus, TNST is physically inspired, as it computes the density transport from a source input smoke to a desired target configuration, allowing control over the amount of dissipated smoke during the stylization process.
 %
%and a differentiable renderer that enables 3D manipulations.
However, TNST faces challenges when dealing with time coherency due to its grid-based discretization. The velocity field computed for the stylization is performed independently for each time step, and the individually computed velocities are recursively aligned for a given window size. Large window sizes are required, rendering the recursive computation expensive while still accumulating inaccuracies in the alignment that can manifest as discontinuities. 
Moreover, transport-based style transfer is only able to advect density values that are present in the original simulation, and therefore it does not inherently support color information or stylizations that undergo heavy structural changes.

%\replace{Thus, in this work, we present an improved algorithm for Transport-based Neural Style Transfer with enhanced temporal coherency. The core contribution of our method is the adoption of a Lagrangian (particle-based) viewpoint over the previous Eulerian (grid-based) discretization. Particle-based systems provide a natural framework for time-coherency, since no recursive alignment of stylization velocities is needed, and \review{changes over time are easy to track in a Lagrangian fashion.}}

Thus, in this work, we reformulate Neural Style Transfer in a Lagrangian setting \add{(see Figure~\ref{fig:overview})}, demonstrating its superior properties compared to its Eulerian counterpart. 
%
In our Lagrangian formulation, we optimize per-particle attributes such as positions, densities and color. This intrinsically ensures better temporal consistency as shown for example in \Fig{colorSmoke}, eliminating the need for the expensive recursive alignment of stylization velocity fields. 
%
The Lagrangian approach reduces the computational cost to enforce time coherency, increasing the speed of results from one day to a single hour.
%
The Lagrangian Style transfer framework is completely oblivious to the underlying fluid solver type. Since the loss function is based on filter activations from pre-trained classification networks, we transfer the information back and forth from particles to the grids, where loss functions and attributes can be jointly updated.
We propose regularization strategies that help to conserve the mass of the underlying simulations, avoiding oversampling of stylization particles. 
%
Our results demonstrate novel artistic manipulations, such as stylization of liquids, color stylization, stylization of multiple fluids, and time-varying stylization. 


%\remove{Moreover, our particle-based approach extends previous TNST - which was limited to support only volumetric smoke data - to further seamlessly stylize liquid simulations. Lastly, the The Lagrangian approach also ensure sharper stylizations which naturally allow colored data, enabling a novel texture transfer from 2D images to 3D volumetric smoke.
%Thus, in this work, we derive a Lagrangian formulation for transport-based neural style transfer. Using particles has unique advantages as the particle motion intrinsically ensures temporal consistency, eliminating the need for recursive alignment of stylization velocities. Moreover, a particle-based viewpoint allows for a unified approach for stylizing smoke and liquids, and enables a wide range of novel artistic effects such as }

%Our contributions can be summarized as

%\review{
%\begin{itemize}
%    \item Generalized framework for stylization of fluid animations in particle-based representation
%    \item Pressure-based penalty for controllable divergence in stylized fluids and re-simulation of Eulerian smoke animation with Lagrangian model
%    \item Differentiable renderer for liquids
%    \item Stylization of Liquids
%    \begin{itemize}
%        \item LazyLiquids (dambreak / liquid sphere drop + wave texture in 2D)
%        \item Surface (Crown to Something like flower? Caustic?)
       % \item Secondary Particles (Spray, Bubble, Foam)
%    \end{itemize}
%    \item Improved differentiable renderer for colorized smoke
%\end{itemize}}

%\add{, follow guideline shapes [ref],  . Either artists. These methods cannot automatically instantiate patterns, and artists }

%\add{Recently, traditional style transfer algorithms were proposed to manipulate smoke data. However }

%\vca{Contextualize Physically-based simulations, artistic manipulations and previous papers that do artistic manipulation. Re-introduce style transfer, the advantages and the limitations. Link the major assumption of this work, overcoming previous limitation. Discuss the new enabled applications. Highlight the major assumption of the work again.}

%
\begin{figure}[h!]
\newcommand*{\mywidth}{0.14}
 \newcommand*{\triml}{70.0}
 \newcommand*{\trimr}{250.0}
%  \newcommand*{\trimr}{350.0}
 \newcommand*{\trimb}{20.0}
 \newcommand*{\trimt}{300}
%  \newcommand*{\trimt}{400}
 \centering
     \includegraphics[width=\mywidth\textwidth]{fig/results/color/lazyfluid_tnst_062_box} 
    \hspace{-26.5px}\includegraphics[width=0.1\linewidth]{fig/results/color/cokeffe}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/lazyfluid_tnst_062_zoom} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/lazyfluid_tnst_066_zoom} 
    %
    \\
    \includegraphics[width=\mywidth\textwidth]{fig/results/color/lazyfluid_lnst_062_box}
    \hspace{-26.5px}\includegraphics[width=0.1\linewidth]{fig/results/color/cokeffe}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/lazyfluid_lnst_062_zoom} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/lazyfluid_lnst_066_zoom} 
    %
    %\\
    % \vspace{1pt}
    %
    \caption{Neural color stylization \cite{christen19color} using the input \emph{Red Canna} applied to a smoke scene with TNST (top) and LNST (bottom). The close-up views (\add{dashed box}, frames 60 and 66) reveal that LNST is more time-coherent than TNST (\add{dashed circle}).}
%}
\label{fig:colorSmoke}
\end{figure}
%

==> LNST arxiv (1)/sec/lagrangianTNST.tex <==

\section{Lagrangian NST}

In contrast to its Eulerian counterpart, the Lagrangian representation uses particles that carry quantities such as the position, density and color value.
Neural style transfer methods compute loss functions based on filter activations from pre-trained classification networks, which are trained on image datasets. Thus, we have to transfer the information back and forth from particles to the grids, where loss functions and attributes can be jointly updated. We take inspiration from hybrid Lagrangian-Eulerian fluid simulation pipelines that use grid-to-particle $\mathcal{I}_{g2p}$ and particle-to-grid $\mathcal{I}_{p2g}$ transfers as
\begin{equation}
\particle{\lambda} = \mathcal{I}_{g2p}(\particle{\vec{x}}, \grid{\lambda}) \;\;\; \text{and} \;\;\; \grid{\lambda} = \mathcal{I}_{p2g}(\particle{\vec{x}}, \particle{\lambda}, h, \grid{\vec{x}}),
\label{eq:peaceAmongWorlds}
\end{equation}
where $\particle{\lambda}$ and $\grid{\lambda}$ are attributes defined on the particle and grid, respectively, $\particle{\vec{x}}$ refers to all particle positions, $\grid{\vec{x}}$ are grid nodes to which values are transferred, and $h$ is the support size of the particle-to-grid transfer. 

Our \gridToParticle~transfer employs a regular grid cubic interpolant, while the particle-to-grid transfer uses standard radial basis functions. Regular Cartesian grids facilitate finding grid vertices around an arbitrary particle position. For this, we extended a differentiable point cloud projector~\cite{insafutdinov2018pointclouds} to arbitrary grid resolution, neighborhood size and custom kernel functions. Given all the neighboring particles \add{$j \in \partial \Omega_{\vec{x}}$} around a grid node \add{$\vec{x}$}, a grid attribute $\grid{\lambda}$ is computed by summing up weighted particle contributions as
%
\begin{equation}
\grid{\lambda}(\vec{x}) = \frac{\sum_{j \in \partial \Omega_{\vec{x}}} \particle{\lambda_j} \; W(||\vec{x}-\particle{\vec{x_j}}||,h)}{\sum_{j \in \partial \Omega_{\vec{x}}}W(||\vec{x}-\particle{\vec{x_j}}||,h)},
\end{equation}
where we chose $W$ to be the cubic B-spline kernel, which is also often used in SPH simulations~\cite{Monaghan2005}:

\begin{equation}
W(r,h)_{\text{cubic}} =
\begin{cases}
\frac{2}{3} - r^2 + \frac{1}{2} r^3, & 0 \leq r \leq 1,\\
\frac{1}{6} (2 - r)^3, & 1 \leq r \leq 2, \\
0, & r > 2.
\end{cases}
\end{equation}
%
%where $W$ is a kernel function.

%Since we employ regular \add{Cartesian} grids, finding the neighborhood of grid vertices around a particle position is very efficient and straightforward \add{and} we extended \remove{and employ} the recent differentiable point cloud projector~\cite{insafutdinov2018pointclouds} for this step. 
%\replace{We have used throughout our examples }

%{For the kernel function $W$ we use} the cubic B-spline kernel 

We now have all the necessary elements to convert the previous Eulerian style transfer (\Eq{tnstSingle}) into a Lagrangian framework. Given a set of Lagrangian attributes $\particle{\vec{\Lambda}}$, the optimization objective for a single frame is
\begin{align}
\particle{\hat{\vec{\Lambda}}} = \argmin_{\particle{\vec{\Lambda}}} \:    \sum_{\theta \in \Theta} \sum_{\particle{\lambda} \in \particle{\Lambda}} w_{\particle{\lambda}} \, \mathcal{L}(\mathcal{R}_\theta(\mathcal{I}_{p2g}(\particle{\vec{x}}, \particle{\lambda}), \, \vec{p}),
\label{eq:LNSTloss}
\end{align}
where $w_{\particle{\lambda}}$ are weights for the losses that include Lagrangian attributes. \add{In case of particle position $\particle{\vec{x}}$ given as the target quantity $\particle{\lambda}$, we use the SPH density $\mathcal{I}_{p2g}(\particle{\vec{x}}) = \sum_{j \in \partial \Omega_{\vec{x}}}{ m_j W(||\vec{x}-\particle{\vec{x}_j}||,h)}$, where $m_j$ represents the mass of the $j$-th particle \cite{splishsplash}.}
Note that our losses are evaluated similarly as in the original Eulerian method, since the gradients computed in image-space also modify grid values ($\grid{\lambda}$). However, these gradients are automatically propagated back to the particles by auto-differentiating the \particleToGrid~ $\mathcal{I}_{p2g}$ function. Thus, our method only reformulates the domain of the optimization, sharing the same stylization possibilities (semantic and content transfers) as in the original TNST.

%The Lagrangian attributes for stylization are example dependent.are scene dependent and , depending on the target example and the type of the simulation. Since the Lagrangian optimization is completely oblivious to the underlying solver, 
Since the Lagrangian optimization is completely oblivious to the underlying solver type, the chosen attributes for creating stylizations can be arbitrarily combined, enabling a wide range of artistic manipulations in different scene setups. 
%
We outline two strategies and demonstrate their impact on the stylization. The first one is particularly suitable for participating volumetric data, which are often simulated with grid-based solvers. It involves optimizing a scalar value carried by the Lagrangian stylization particles by \Eq{LNSTloss}. For most of our smoke scenes, this scalar value is the density, though it can also be the color or emission. The regularization term
%
%We outline two strategies \revise{used throughout all our examples}. The first strategy is more suitable for participating volumetric data, and it involves optimizing a scalar value carried by the Lagrangian particles by \Eq{LNSTloss}. \revise{For most of our smoke scenes, this scalar value is the density, though it can also be the color or emission values. Particularly for smoke scenes, we add a regularization term for the Lagrangian density attribute} 
%
\begin{equation}
\mathcal{L}({\particle{\lambda}})_\rho =  (\sum {\Delta \particle{\lambda}})^2 - \sum \log {||\Delta \particle{\lambda}||_1}
\label{eq:densityConserv}
\end{equation}
reinforces the conservation of the original amount of smoke. It minimizes the total net smoke change, preventing the stylization to undesirably fade out particles and keeping changes non-zero by minimizing cross-entropy loss at the same time. \Fig{regularizer_density} demonstrates the impact of different regularizer weights.
%
\begin{figure}[h!]
\newcommand*{\mywidth}{0.1}
 \newcommand*{\triml}{370.0}
 \newcommand*{\trimr}{340.0}
 \newcommand*{\trimb}{30.0}
 \newcommand*{\trimt}{80}
 \centering
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip,
    width=\mywidth\textwidth]{fig/results/TNST_LNST/net_new_105.jpg}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, 
    width=\mywidth\textwidth]{fig/method/regularizer/net_d8_105.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/method/regularizer/net_d7_105.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/net_gt_105.jpg}
   % \hspace{-27.7px}\includegraphics[width=0.1\linewidth]{fig/results/liquids/pattern1.png}
    \caption{
    Different weights for the density regularization show the trade-off between pronounced structures and conservation of mass. The images on the left show results with zero, low, and high weights, respectively, and the right image is the ground truth.
    }
%}
\label{fig:regularizer_density}
\end{figure}
%

The second strategy is suitable if the underlying fluid solver is particle-based or hybrid, which is often the case for liquids.
For these simulations, we can define particle position displacements as the optimized Lagrangian attributes. However, generating stylizations by modifying particle displacements may cause cluttering or regions with insufficient particles. The regularization penalizes irregular distribution of particle positions 
%\remove{, common in position-based simulations \cite{Macklin2013}} 
and is defined as 
\begin{align}
\mathcal{L}(\particle{\vec{x}})_{\Delta x} = ||\mathcal{I}_{p2g}(\particle{\vec{x}}) - \grid{\rho_0}||_2 ^ 2,
\label{eq:positionUpdato}
\end{align}
where $\grid{\rho_0}$ corresponds to the rest density for cells that contain particles, and is zero otherwise. 
Note that \Eq{positionUpdato} does not account for the particle deficiency near fluid surfaces. This could be addressed by adding virtual particles \cite{Schechter2008} or applying (variants of) the Shepard correction to the kernel function \cite{Reinhardt2019}.
We show the impact of this regularizer on the particle sampling in \Fig{regularizer_position}, highlighting the trade-off between uniform distribution and stylization strength.
%
\begin{figure}[h!]
\newcommand*{\mywidth}{0.095}
 \newcommand*{\triml}{370.0}
 \newcommand*{\trimr}{370.0}
 \newcommand*{\trimb}{0.0}
 \newcommand*{\trimt}{70}
 \centering
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip,
    width=\mywidth\textwidth]{fig/results/liquids/buckling_spiral_87.jpg}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, 
    width=\mywidth\textwidth]{fig/method/regularizer/buckling_spiral_pr4_87.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/method/regularizer/buckling_spiral_pr6_87.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/liquids/gt_buckling_87.jpg}
   % \hspace{-27.7px}\includegraphics[width=0.1\linewidth]{fig/results/liquids/pattern1.png}
    \caption{
    Different weights for the position regularization show the trade-off between pronounced structures and uniform sampling. The images on the left show results with zero, low, and high weights, respectively, and the right image is the ground truth.
    }
%}
\label{fig:regularizer_position}
\end{figure}
%





We notice that both regularizations in \Eq{densityConserv} and \Eq{positionUpdato} are different incarnations of the mass conservation property commonly used in fluid simulations. In TNST, mass conservation is enforced by decomposing the stylization velocities into their irrotational and incompressible parts, which can be optimized independently. 
Both techniques enable a high degree of artistic control over the content manipulation.


%On the next subsections we will discuss how to convert Eulerian smoke simulations into an efficient particle representation and how to implement temporal coherency in the proposed Lagrangian framework.

%In TNST, input fields are composed of irrotational and incompressible parts for divergence control. We can use~\Eq{densityConserv}~and~\Eq{positionUpdato} as a regularizer for incompressibility of quantities and particle distributions, respectively. Do we need to show the effect of \Eq{densityConserv}? Then a comparison figure will be added

%\replace{One shortcoming of employing our Lagrangian Neural Style Transfer is that most of smoke solvers discretize the volumetric domain with grids. Trying to approximate the original grid-based density by sampling particles and advecting them poses problems.}

\subsection{An Efficient Particle-Based Smoke Re-Simulation}

%\vca{I think the previous structure was fine. Maybe we can say that this makes the process imperceptible for the end-user.}
%\reviewWComment{The Lagrangian formulation requires the approximation of grid-based density by sampling particles and advecting them, which comes with a few challenges.}
%\replace{First, we aim at a sparse and efficient particle representation, ideally sampling only one particle per \replace{cell}{voxel}. As a comparison, hybrid liquid simulations usually sample 8 particles per \replace{cell}{voxel} to properly capture momentum conservation \cite{Zhu2005}. 
%}
{
%\replace{For grid-based simulations}
%{Since the simulation inputs are represented as grids,}
\add{If the input is a grid-based simulation,} we have to sample and re-simulate particles. We can use a sparse representation with only one particle per voxel, in constrast to hybrid liquid simulations that usually sample 8 particles per voxel to properly capture momentum conservation \cite{Zhu2005}.
}
Combining a low number of particles with a position integration algorithm that accumulates errors over time will yield irregularly distributed particles \cite{Ando2011}. This manifests in a rendered image as smoke with overly dense or void regions. 
%\bs{I would remove the following sentence and directly show the equation}\revise{Apart from that, the density value individually carried by each particle which minimizes the discrepancy between the Eulerian and Lagrangian representations is unknown. Keeping the per-particle density constant by simply assuming that the material derivative to be $\frac{Dp}{Dt} = 0$ would not properly capture how the density changes \replace{for}{as} Lagrangian structures evolve}. 
We therfore solve the following optimization problem
\begin{align}
\particle{\hat{\vec{x}}}, \particle{\hat{\rho}} = \argmin_{{\particle{\vec{x}}, \particle{\rho}}} \sum_t ||\mathcal{I}_{p2g}(\particle{\vec{x}}_t, \particle{\rho_t}) - \grid{\rho_t}||_2 ^ 2.
\label{eq:resimulationOptimization}
\end{align}

%We want to thus minimize the reconstruction error as follows:\ This problem is severely unconstrained, and since considers time-varying data, highly challenging to be solved. 
%
The optimization problem presented above is not only severely under-constrained but also has a time-varying objective term, and optimizing for \Eq{resimulationOptimization} is challenging if tackled jointly for both particle positions $\particle{\vec{x}}$ and densities $\particle{\rho}$. Thus, we use a heuristic approach for solving this optimization, subdividing it into two steps, position optimization and multi-scale density update (\Sec{multiscale}). Firstly, we minimize the irregular distribution of particle positions by employing a position-based update, optimizing particle distributions using \Eq{positionUpdato} as objective.
%\begin{align}
%\particle{\hat{\vec{x}}} = \argmin_{\particle{\vec{x}}} ||\mathcal{I}_{p2g}(\particle{\vec{x}}, \rho_0) - \grid{\rho_0}|| ^ 2,
%\label{eq:positionUpdato}
%\end{align}
%where $\grid{\rho_0}$ \replace{represents the density field filled with a rest density value where particle exists (zero elsewhere).}{corresponds to the %rest density for cells that contain particles, and is zero otherwise.}
%
 The distribution of the particles is optimized per frame and serves as an input for optimizing subsequent frames, enabling temporally coherent position updates. \Eq{positionUpdato} can be automatically computed by our fully differentiable pipeline.% \review{(see Section XXX)}.

%While our approach does not guarantee the optimality of the solution, it yields results that are very close to the original grid-based densities as shown in image. 
\subsubsection{Multi-scale Density Representation}
\label{sec:multiscale}
%\bs{I used the term multi-scale stylization using cascading residulas since it does entirely correspond to Laplacian pyramids, not sure if this makes sense}

In addition to the position update, we also compute smoke densities individually carried by the particles to further eliminate small gaps that may appear due to the sparse discretization, further enhancing the solution of \Eq{resimulationOptimization}. Owing to the low number of sampled particles and the mismatches between grid and particle transfers, carrying a constant density will either produce grainy (\Fig{resim_compare}, (b)) or diffuse (\Fig{resim_compare}, (c)) volumetric representations, depending on if particle re-distribution (\Eq{positionUpdato}) is applied or not.
A simple approach is to interpolate density values directly from the grid over time. Larger kernel sizes could be used to remedy sparse sampling, but would excessively smooth structures and degrade quality.
% 
%We show a comparison of different parameter configurations in \review{\Fig{resim_compare}}.
%
\begin{figure}[t!]
    \centering
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, width=0.128\textwidth]{fig/method/resim/5_gt}}{\scriptsize{(a)}}
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, width=0.128\textwidth]{fig/method/resim/0_no_dist_const_den}}{\scriptsize{(b)}}
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, width=0.128\textwidth]{fig/method/resim/1_dist_const_den}}{\scriptsize{(c)}}
    \\
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, width=0.128\textwidth]{fig/method/resim/2_no_dist_s1}}{\scriptsize{(d)}}
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, 
    width=0.128\textwidth]{fig/method/resim/3_dist_s1}}{\scriptsize{(e)}}
    \stackunder{\includegraphics[trim = 0px 0px 0px 0px, clip, width=0.128\textwidth]{fig/method/resim/4_dist_s3}}{\scriptsize{(f)}}
    %
    \vspace{-3mm}
    \caption{
    %
    Comparison of different re-simulation strategies. (a): ground truth density, (b): constant density carried by particles, (c): (b) with redistribution by \Eq{positionUpdato}, (d): single-scale sampled density, (e): (d) with redistribution, (f): multi-scale \add{($n_s=3$)} sampled density with redistribution (final method).
    }
    \label{fig:resim_compare}
    \vspace{-5px}
\end{figure}
%

%The wide number of choices for  different types of kernels and their configurable support sizes creates a problem for finding the optimal parameters. Additionally, when the heavily undersampled particle distribution transfers its information using \particleToGrid $\mathcal{I}_{p2g}$ tends to act as a low pass filter, blurring the details that particles may carry when \gridToParticle transfers information to the grids.}
%We notice, however, that the way that particles are represented on the grid heavily depend on the \particleToGrid $\mathcal{I}_{p2g}$ operation and its configuration. 

We take inspiration from Laplacian pyramids, where distinct grid resolution levels are treated separately. In our case, we compute residuals of different support kernel sizes of the \particleToGrid~transfer. This efficiently captures both low- and high-frequency information, covering potentially empty smoke regions while also providing sharp reconstruction results. The residual computation of kernels of varying support sizes is synergistically coupled with matching grid resolutions, which creates an efficient multi-scale representation of the smoke.

%frequency information that was not entirely optimized in the previous position update step, covering possible empty smoke regions. For capturing the high-frequency details, we transfer to particles the difference between \particleToGrid~transfers that have distinct kernel support radius. 

%while also capturing high-frequency information at a substantially low performance decrease, We couple this approach with also varying the grid resolution for a performance speed-up, since bigger kernels tend to oversmooth the solution, and the additional degrees of freedom used by higher resolution grid would be unused.
The multi-scale reconstruction works as follows: we first sample grid densities to the particles. This represents the smoke low-frequency information, which we interpolate to the particle variables $\particle{\rho_0}$. The variables above the first level (\eg $\particle{\rho_1}, \particle{\rho_2}$) will carry residual information computed between subsequent levels. The Lagrangian representations vary between each level because they perform \gridToParticle~transfers with progressively reduced kernel support sizes. To compare residuals between Lagrangian representations, we make use of \particleToGrid~transfers, which act as a low-pass filter, similarly to blurring operations of Laplacian pyramids. This process is performed until the original grid resolution is matched. Our multi-scale density representation is summarized in \Algo{densitySample}.
% we first downscale the original grid-based smoke simulation to a pre-specified number of pyramid levels. For example, if the volumetric smoke has $n$ cells, the coarsest resolution of its 4-level pyramid will have $n \cdot 2^{-4}$ cells. This represents the smoke low-frequency information, which we interpolate to the particle variables $\particle{\rho_0}$. The variables above the first level (\eg $\particle{\rho_1}, \particle{\rho_2}$) will carry residual information computed between subsequent levels. \addComment{what does it mean representation varies? does this refer to the stylized structure?} \review{The Lagrangian representations vary} \review{between each level} because they perform \gridToParticle~transfers with progressively reduced kernel support sizes. To compare residuals between Lagrangian representations, we make use of \particleToGrid~transfers, which are combined with upsampling and blurring operations, similarly to Laplacian pyramids. This process is performed until the original grid resolution is matched. Our multi-scale density representation is summarized in \Algo{densitySample}.
\Fig{resim_compare} illustrates the impact of using a single scale without (d) and with (e) particle re-distribition (\Eq{positionUpdato}). The multi-scale result with re-distribution (f), which corresponds to our final method, has a higher PSNR (31.89) than its single-scale counterpart (31.39) and is very close to the ground truth (a).

%\add{In order to reconstruct grid densities from the previously optimized positions, we perform a \gridToParticle~transfer from the original smoke sources to the particles. Since this represents the ground-truth smoke that we are trying to approximation, we use this information as the low frequency information carries by the particles. This information gets transferred with a \particleToGrid approach using a large support kernel radius to ensure that we cover void regions. However, the large kernel support will produce a blurred grid representation. Hence, on the next step, we decrease the kernel radius support - employing a factor of 2 but an arbitrary reduction could be also used - and. This process is summarized in \Algo{densitySample} }

% \begin{algorithm}
% \SetAlgoLined
% \KwData{Particle positions \(\particle{\vec{x}} \) optimized by \Eq{positionUpdato} \\
%         Original grid-based smoke simulation \(\grid{\rho}\) \\
%         Dimensions of original sim $n$ \\
%         Number of pyramid subdivisions $n_s$ \\
%         Coarsest support kernel radius $r$ }
% \KwResult{Multi-scale residual densities representations stored in Lagrangian attributes}
% \BlankLine
% \(\particle{\rho_0} \leftarrow \mathcal{I}_{g2p} (\particle{\vec{x}}, \grid{\rho}) \) \\
% \tcp{\(\grid{\rho_*} \) has initial dimensions \(n \cdot 2^{-n_s}\) }
% \(\grid{\rho_*} \leftarrow \mathcal{I}_{p2g} (\particle{\vec{x}}, \particle{\rho_0}, r) \)\\
% \For{\(i \leftarrow 1 \) \KwTo \(n_{s}\)}{
%     \( r \leftarrow \frac{r}{2} \) \\
%     \(\particle{\rho_i} \leftarrow \mathcal{I}_{g2p} (\particle{\vec{x}}, \mathcal{I}_{p2g} (\particle{\vec{x}}, \particle{\rho_{i- 1}}, r) - \mathcal{B}(\mathcal{U}(\grid{\rho^*},~2)))\) \\
%     \(\grid{\rho_*} \leftarrow \grid{\rho^*} + \mathcal{I}_{p2g} (\particle{\vec{x}}, \particle{\rho_i}, r)\) \\
% }
% \caption{Multi-scale Density Reconstruction}
% \label{algo:densitySample}
% \end{algorithm}


\begin{algorithm}
\SetAlgoLined
\KwData{Particle positions \(\particle{\vec{x}} \) optimized by \Eq{positionUpdato}\\
        Original grid-based smoke simulation \(\grid{\rho}\) \\
        Grid node positions $\grid{\vec{x}}$ \\
        Coarsest support kernel radius $r$ \\
        Number of pyramid subdivisions $n_s$}
\KwResult{Multi-scale residual density \(\particle{\rho}\) stored on particles}
\BlankLine
\(\particle{\rho_0} \leftarrow \mathcal{I}_{g2p} (\particle{\vec{x}}, \grid{\rho}) \) \\
\(\grid{\rho_*} \leftarrow \mathcal{I}_{p2g} (\particle{\vec{x}}, \particle{\rho_0}, r, \grid{\vec{x}}) \)\\
\For{\(i \leftarrow 1 \) \KwTo \(n_{s}\)}{
    \(\grid{\rho_*} \leftarrow \grid{\rho}- \grid{\rho_*}\)\\
    \(\particle{\rho_i} \leftarrow \mathcal{I}_{g2p} (\particle{\vec{x}}, \grid{\rho_*})\) \\
    \( r \leftarrow \frac{r}{2} \) \\
    \(\grid{\rho_*} \leftarrow \grid{\rho_*} + \mathcal{I}_{p2g} (\particle{\vec{x}}, \particle{\rho_i}, r, \grid{\vec{x}})\) \\
}
\caption{Multi-scale Density Reconstruction}
\label{algo:densitySample}
\end{algorithm}



% Interpolate on first level
% Splat to grid
% Compute residuals
% Kernel support = K/2

%The type of the kernel function and the its radius support will   

%The second part of the 

%While this could be done for the Eulerian setting, this would require the alignment of velocity fields in different levels, making the algorihm even slower.

%Contrary to traditional laplacian pyramid we dont blur after doing \particleToGrid. This happens because the particle to grid operation already works as blurring filter. Additionally, the next level of particle splatting will only represent what the previous level was unable to capture. 

\subsection{Temporal coherency}
The major advantage of our Lagrangian discretization is the inexpensive enforcing of temporal coherency. Since quantities are carried individually per particle, it is intrinsically simple to track how attributes change over time. Neural style gradients are computed on the grid and need to be updated once the neighborhood of a particle changes. To ensure smooth transitions, we apply a Gaussian filter over the density changes of a particle, as shown in \Fig{babyDensities}.
Besides being sensitive to density neighborhood changes, stylization gradients are also influenced by the density carried by the particle itself (\Sec{multiscale}).
%
\begin{figure} [h!]
  \centering
  \includegraphics[width=0.4\textwidth]{fig/method/lagrangianDensities}
  \caption{Particle density (circles) variation for a single particle over time. Temporal coherency is enforced by smoothing density gradients used for stylization from adjacent frames.}
  \label{fig:babyDensities}
\end{figure}

% moved to sec3
%\begin{figure} [h!]
%  \centering
 % \includegraphics[width=0.45\textwidth]{fig/method/tnst_align.png}
 % \caption{Recursive temporal alignment of a window size 9 in TNST.}
%  \label{fig:tnstalign}
%\end{figure}


%also changes to match the original grid-based smoke simulation These density changes will also create stylization gradients on image space 


To further improve efficiency, and in contrast to TNST, we can keyframe stylizations, i.e., apply stylization to keyframes and interpolate particle attributes in-between. In practice, we reduced the stylization frames by a factor of 2 at max, but more drastic approximations could be used. Sparse keyframes still show temporally smooth transitions, but quality is degraded. Nevertheless, sparse keyframing would still be useful for generating quick previews of the simulation. The impact of sparse keyframing (every 10 frames) is shown in \Fig{keyframe}.
%
\begin{figure}[t!]
 \centering
    \includegraphics[trim=0 0 900 0,clip, width=0.435\textwidth]{fig/method/keyframe/seq.jpg}
    \caption{
    Stylization of every frame (left three images) versus keyframed stylization every 10 frames (images on the right). %\replace{\add{It is still visually similar to the left one.}}
    \add{Sparse keyframing is visually similar and can be useful for quick previews.}
    }
%}
\label{fig:keyframe}
\end{figure}
%

%\add{The impact of keyframing on the performance is discussed in \Sec{}.}



%\review{The losses computed from the Neural Style transfer generate artistic manipulations that violate underlying equations. As the Lagrangian formulation does not indirectly manipulate attributes by advection, as TNST, we do not enforce incompressibility constraints. However, we will show in section XX, we add to our optimization a regularization to reduce material dissipation.  Additionally, we can add regularization terms that will penalize density changes removing completely the amount of smoke. One of those changes is just adding  As each particle tracks only its local values, still, we have}


==> LNST arxiv (1)/sec/related_work.tex <==
\section{Related Work}

\emph{Lagrangian Fluids} have become popular for simulating incompressible fluids and interactions with various materials. 
Since the introduction of SPH to computer graphics \cite{Desbrun1996,Muller2003}, various extensions have been presented that made it possible to efficiently simulate millions of particles on a single desktop computer. Accordingly, particle methods reached an unprecedented level of visual quality, where fine-scale surface effects and flow details are reliably captured. To enforce incompressibility, the original state equation based method \cite{Monaghan2005,Becker2007} has been replaced by pressure Poisson equation (PPE) solvers using either a single source term for density invariance \cite{Solenthaler2009,Ihmsen2014} or two PPEs to additionally account for divergence-free velocities \cite{Bender2015}. Solvers closely related to PPE have been presented, such as Local Poisson SPH \cite{He2012}, Constraint Fluids \cite{Bodin2012} and Position-based Fluids \cite{Macklin2013}. Boundary handling is computed with particle-based approaches that sample boundary geometry (e.g. \cite{Gissler2019}) or implicit methods that typically use a signed distance field (e.g. \cite{Koschier2017}). Extensions include highly viscous fluids (e.g. \cite{Peer2015}), and multiple phases and fluid mixing (e.g. \cite{Ren2014}).
An overview of recent developments in SPH can be found in the course notes of Koschier et al. \shortcite{Koschier2019}.

\vspace{0.1cm}

\emph{Hybrid Lagrangian-Eulerian Fluids} combine the versatility of the particles representation to track transported quantities with the capacity of grids to enforce incompressibility. Among popular approaches, the Fluid Implicit Particle Method (FLIP) \cite{Brackbill1988} was first employed in graphics to animate sand and water \cite{Zhu2005}. Due to its ability to accurately capture sub-grid details it has been widely adopted for liquid simulations, being extended to animation of turbulent water \cite{Kim2007}, coupled with SPH for modelling small scale splashes \cite{Losasso2008}, improved for efficiency \cite{Ando2013, Ferstl2016}, used in fluid control \cite{Pan2013}, and enhanced with better particle distribution \cite{Ando2011, Um2014}. 
\add{The Material Point Method (MPM) \cite{stomakhin2013} was used to simulate a wide class of solid materials \cite{jiang2016material}.} 
Recent work on hybrid approaches extended the information tracked by the particles by affine \cite{Jiang2015} and polynomial \cite{Fu2017} transformations. For a thorough discussion of hybrid continuum models, we refer to Hu et al. \shortcite{Hu2019}.

%The APIC method extends Lagrangian tracking of velocities to also track affine transforms. } In this way the method is better able to conserve rotational and shearing modes, usually lost by the overdissipative nature of the interpolations of the particle in cell approach while also keeping the stability of ble. 

\vspace{0.1cm}

\emph{Patch-based Appearance Transfer} methods compute similarities between source and target datasets in local neighborhoods, modifying the appearance of the source by transferring best-matched features from the target dataset. Kwatra et al. \shortcite{Kwatra2005} employ local similarity measures in an energy-based optimization, enabling texture patches animated by flow fields. This approach was further extended to liquid surfaces \cite{Kwatra2006, Bargteil2006}, and improved by modifying the texture based on visually salient features of the liquid mesh \cite{Narain2007}. Jamri\v{s}ka et al. \shortcite{jamrivska2015lazyfluids} improved previous work with better temporal coherency and matching precision for obtaining high-quality 2D textured fluids. Texturing liquid simulations was also implemented in a Lagrangian framework by using individually tracked surface patches \cite{Yu2011, Gagnon2016, Gagnon2019}. Image and video-based approaches also take inspiration from fluid transport. Bousseau et al. \shortcite{Bousseau2007} proposed a bidirectional advection scheme to reduce patch distortions. Regenerative morphing and image melding techniques were combined with patch-based tracking to produce in-betweens for artist-stylized keyframes \cite{browning2014stylized}. Recent advances in patch-based appearance transfer often rely on evaluating the underlying 3D geometric information; examples include improving template matching by a novel similarity measure \cite{Talmi2016}, patch matching for illumination effects \cite{Fiser2016}, extensions to texture mapping \cite{Bi2017} and intricate texture motifs \cite{Diamanti2015}. While these approaches were successful in 2D settings and for texturing liquids, they cannot inherently support 3D volumetric data.

\vspace{0.1cm}

\emph{Velocity Synthesis} methods augment flow simulations with velocity fields, which manipulate or enhance volumetric data. Due to the inability of pressure-velocity formulations to properly conserve different energy scales of flow phenomena, sub-grid turbulence~\cite{kim2008wavelet, Schechter2008, Narain2008} was modelled for better energy conservation. These approaches were extended to model turbulence in the wake of solid boundaries \cite{Pfaff2009}, liquid surfaces~\cite{kim2013closest} and example-based turbulence synthesis \cite{sato2018example}. In order to merge fluids of different simulation instances \cite{Thuerey2016} or separated by void regions \cite{sato2018example}, velocity fields where synthesized by solving an unconstrained energy minimization problem. Lastly, the Transport-based Neural Style Transfer (TNST) \cite{Kim2019} can also be seen as a velocity synthesis method: at each time-step, the method optimizes a velocity field that transports the smoke towards a desired stylization.

%transferred turbulence from a source simulation to a target one similarly to patch-based appearance transfer methods  
%Ma et al. \shortcite{ma2009motion} synthesized velocity fields with example-based textures for artistic manipulations, but their method is limited to simple \twoD~patterns.

\vspace{0.1cm}

\emph{Machine Learning \& Fluids} 
was first introduced to graphics by Ladick\'{y} et al. \shortcite{Ladicky2015}. They used Regression Forests to predict positions of fluid particles over time, resulting in a substantial performance gain compared to traditional Lagrangian solvers.
CNN-based architectures were employed in Eulerian-based solvers to substitute the pressure projection step \cite{Tompson2016, Yang2016} and to synthesize flow simulations from a set of reduced parameters \cite{Kim2019deep}. An LSTM architecture \cite{Wiewel2018} predicted changes on pressure fields for multiple subsequent time-steps, speeding up the pressure projection step. Differentiable fluid solvers \cite{Schenck2018, Hu2018, Hu2020DiffTaichi, Holl2020} have been introduced that can be automatically coupled with \add{deep learning} architectures and provide a natural interface for image-based applications. Patch-based \cite{Chu2017} and GAN-based \cite{xie2018tempogan} fluid super-resolution enhance coarse simulations with rich turbulence details, while also being computationally inexpensive. While these approaches produce detailed, high-quality results, they do not support transfer of arbitrary smoke styles.

\vspace{0.1cm}

\emph{Differentiable Rendering and Stylization} is used in Neural Style Transfer algorithms to transfer the style of a source image to a target image by matching features of a pre-trained classified network \cite{gatys2016}. However, stylizing 3D data requires a differentiable renderer to map the representation to image space. Loper and Black \shortcite{Loper2014} proposed the first fully differentiable renderer with automatically computed derivatives, while a novel differentiable volume sampling was implemented by Yan et al. \shortcite{Yan2016}. Raster-based differentiable rendering for meshes for stylization with approximate \cite{kato2018neural} and analytic \cite{liu2018paparazzi} derivatives was proposed to approximate visibility changes and mesh filters, respectively. A cubic stylization algorithm \cite{Liu2019} was implemented by minimizing a constrained energy formulation and employed to mesh stylization. Closer to our work, Kim et al. \shortcite{Kim2019} defines an Eulerian framework for a transport-based neural style transfer of smoke. Their approach computes individually stylized velocity fields per-frame, and temporal coherence is enforced by aligning subsequent stylization velocity fields and performing smoothing. 
%
We compare the Eulerian approach with our method in the subsequent sections. 
For an overview on differentiable rendering and neural style transfer we refer to Yifan et al. \shortcite{Yifan2019} and Jing et al. \shortcite{jing1705neural}, respectively.

%There is a growing interest on differentiable ray marching and path tracers and Li et al. \shortcite{Li2018} introduces the first general-purpose differentiable ray tracer by removing discontinuities by directly sampling Dirac delta functions, while a differentiable path-tracer for inverse volumetric rendering with joint estimation of geometry was proposed by Velinov et al. \shortcite{Velinov2018}

%\add{{Neural Style Transfer} algorithms transfer the style of a source image to a target image by matching features of a pre-trained classified network \cite{gatys2016, gatys2017}. Originally, the process of matching features was done by solving an inefficient unconstrained minimization problem, and most of modern approaches train Deep CNNs to achieve interactive results. Johnson et al. \shortcite{Johnson2016Perceptual} used perceptual losses to train a network for stylization, Ulyanov et al. \shortcite{Ulyanov2016} employed instance-normalization instead of batch-normalization for improved results, and a hierarchical multi-modal CNN \cite{Wang2016} was proposed to capture styles across distinct texture scales. Several works implemented neural style transfer for video sequences. Ruder et al. \shortcite{ruder2016artistic} addressed temporal coherency issues considering occluded regions and long term correspondences, \addComment{\vca{add more temporal coherence references}}.}

%\reviewWComment{\emph{Neural Style Transfer} is the process of rendering image content in different styles by exploring CNNs. The seminal work of Gatys et al. \shortcite{gatys2016} was the first to transfer painting styles to natural images. Their model relies on extracting the content of an image by measuring filter responses of a pre-trained CNN, while modelling the style as summary feature statistics. The network's filter responses decompose the image complexity into multiple levels, ranging from low-level features to high-level semantics. Given a target style, NST approaches optimize CNN feature distributions of a source image style, while keeping its original content. Ruder et al. \shortcite{ruder2016artistic} implemented style transfer for video sequences, addressing temporal coherency issues due to occluded regions and long term correspondences, while Mordvintsev et al. \shortcite{mordvintsev2018differentiable} discuss the impact of different choices of image parameterizations for NST. For a detailed review of NST methods we refer to~\cite{jing1705neural}.}{\vca{Rewrite this adding more references. Copy paste from TNST}}

%\empth{Hybrid Eulerian-Lagrangian fluid models} \addComment{\vca{We have to expand this with FLIP, APIC, PolyPIC, MPM, etc.}} \bk{particle-based fluid simulations: sph, pbd, a particle-based method for preserving fluid sheets, hybrid sph, etc.}

%\bk{new differentiable rendering papers (see siggraph asia 2019 differentiable rendering section + Mitsuba2). Differentiable Surface Splatting for Point-based Geometry Processing~\cite{yifan2019dss}. SDFDiff: Differentiable Rendering of Signed Distance Fields for 3D Shape
%Optimization.  We adopted the discretization code of differentiable point cloud \cite{insafutdinov2018pointclouds} for density splatting with sph kernels.}

%\bk{stylizations/optimization on geometry, liquid, etc. than image (see siggraph asia 2019 geometry with style section}

==> LNST arxiv (1)/sec/results.tex <==
\section{Results}
% ~\cite{tensorflow2015-whitepaper} too long
We implemented the method with the \emph{tensorflow} framework and computed results on a TITAN Xp GPU (12GB). We used \emph{mantaflow} \cite{mantaflow} for smoke scene generation, a \threeD~smoke dataset from Kim et al. \shortcite{Kim2019} for comparisons with TNST, a \twoD~smoke dataset from Jamri\v{s}ka et al.~\shortcite{jamrivska2015lazyfluids} for color stylization, \emph{SPlisHSPlasH}~\cite{splishsplash,Koschier2019} for liquid simulations and \emph{Houdini} for rendering.



\paragraph{Performance}
Using particles for stylization eliminates the need for recursively aligning stylization velocities from subsequent frames, which notably improves the computational performance.
In combination with our sparse particle respesentation for smoke (1 particle per cell), simulations of size $200\times300\times200$ can now be stylized within an hour instead of a day (TNST). The computation time per frame is 0.66 minutes for the Smoke Jet scene shown in \Fig{tnst_lnst}, which is a speed-up of a factor of 20.41 compared to TNST. This improvement allows artists to more easily test different reference structures (input images) and hence renders neural flow stylization better applicable in production environments. \Tab{performance} gives an overview of the timings and parameters for the individual test scenes. 
Keyframing (every other frame) was applied to the Smoke Jet (\Fig{tnst_lnst}) and Double Jets (\Fig{multifluid}) examples. 
%
\begin{table}[h!]
\caption{Performance table.}
\vspace{-5pt}
\begin{tabular}{p{2.7cm} ccccccc}
\hline
\small{Scene} & \small{Resolution} & \# \small{Particles} & \small{Time (m/f)}
\tabularnewline \hline
\small{Moving Sphere} \footnotesize{(Fig.~\ref{fig:spheretest})} & $192\times192\times192$ & 237K & 0.8\\
\small{Smoke Jet} \footnotesize{(Fig.~\ref{fig:tnst_lnst})} & $200\times300\times200$ & 1.2M & 0.66\\
\small{Double Jets} \footnotesize{(Fig.~\ref{fig:multifluid})} & $200\times200\times200$ & 2M/2M & 0.45\\
\small{Chocolate} \footnotesize{(Fig.~\ref{fig:chocolate})} & $200\times200\times200$ & 80K & 0.05\\
\small{Colored Smoke} \footnotesize{(Fig.~\ref{fig:colorSmoke})} & $800\times800$ & 136K & 1.21\\
\small{Dam Break} \footnotesize{(Fig.~\ref{fig:color})} & $512\times1024$ & 23K & 0.58\\
\small{Double Dam} \footnotesize{(Fig.~\ref{fig:colormix})} & $512\times1024$ & 31K/8K & 0.65
\tabularnewline \hline
\end{tabular}
\label{tab:performance}
\vspace{-5pt}
\end{table}
%


%\begin{table*}[h!]
%\caption{Performance table.}%into account it as a valid compression.}
%\vspace{-5pt}
%\begin{tabular}{p{3.2cm} ccccccc}
%\hline
%\small{Scene} & \small{Resolution} & \# \small{Particles} & \# \small{Frames} & \# \small{Key Frames} & \small{Comp. Time (m/f)} & \small{Speed up}
%\tabularnewline \hline
%\small{Moving Sphere} \footnotesize{(Fig.~\ref{fig:spheretest})} & $192\times192\times192$ & 237K & 20 & 1 & 0.8 & 3.75\\
%\small{Smoke Jet} \footnotesize{(Fig.~\ref{fig:tnst_lnst})} & $200\times300\times200$ & 1.2M & 120 & 2 & 0.66 & 20.41\\
%\small{Colliding Jets} \footnotesize{(Fig.~\ref{fig:multifluid})} & $200\times200\times200$ & 2M/2M & 120 & 2 & 0.45 & -\\
%\small{Chocolate} \footnotesize{(Fig.~\ref{fig:chocolate})} & $200\times200\times200$ & 80K & 120 & 1 & 0.05 & -\\
%\small{Colored smoke} \footnotesize{(Fig.~\ref{fig:colorSmoke})} & $800\times800$ & 136K & 180 & 1 & 1.21 & 1.22\\
%\small{Dam Break} \footnotesize{(Fig.~\ref{fig:color})} & $512\times1024$ & 23K & 200 & 1 & 0.58 & -\\
%\small{Double Dam Break} \footnotesize{(Fig.~\ref{fig:colormix})} & $512\times1024$ & 31K/8K & 200 & 1 & 0.65 & -
%\tabularnewline \hline
%\end{tabular}
%\label{tab:performance}
%\vspace{-5pt}
%\end{table*}



\paragraph{Time-coherency}
To illustrate the benefit of the Lagrangian formulation, we use a simple test scene where we initialize a smoke sphere with a uniform density. We then move the smoke artificially to the right, and apply the neural stylization to every frame of the sequence. We compare the results of LNST and TNST for different time instances in \Fig{spheretest}. 
The top row shows the results of TNST. It can be seen that TNST is not able to preserve constant stylized textures in regions where the density function does not change. This is due to the recursive alignment of stylization gradients, which accumulate errors especially for bigger window sizes.
The second row shows the corresponding results with LNST, demonstrating consistent stylization over time since gradients are constant. Also when applied a shearing deformation to the sphere, as shown in the third row, strucutures remain coherent. If an artist prefers to have changing structures in such situations, noise can be added to the densities carried by the particles, which in turn will induce stylization gradients as shown in the last row.
 %
\begin{figure}[t!]
% \newcommand*{\mywidth}{0.115}
%  \newcommand*{\triml}{370.0}
%  \newcommand*{\trimr}{370.0}
%  \newcommand*{\trimb}{0.0}
%  \newcommand*{\trimt}{0}
 \centering
 \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/t_trans/000}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/t_trans/009}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/t_trans/019}\\
\includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_trans/000}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_trans/009}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_trans/019}\\
\includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_shear/000}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_shear/009}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_shear/019}\\
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_noise/000}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_noise/009}\hspace{-1px}
    \includegraphics[trim={0 45 40 45}, clip,
    width=0.13\textwidth]{fig/method/tempo/l_noise/019}
%  \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/t_trans/000.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/t_trans/009.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/t_trans/019.jpg}\\
% \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_trans/000.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_trans/009.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_trans/019.jpg}\\
% \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_shear/000.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_shear/009.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_shear/019.jpg}\\
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_noise/000.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_noise/009.jpg}\hspace{-1px}
%     \includegraphics[trim={10 20 0 20}, clip,
%     width=0.14\textwidth]{fig/method/tempo/l_noise/019.jpg}

    \caption{
    Selected frames of a stylized moving smoke sphere. From top to bottom: TNST with structures changing over time, LNST with temporally coherent structures, LNST result with applied shearing, and LNST result with noise-added density inducing style variation over time.
    }
%}
\label{fig:spheretest}
\end{figure}

\paragraph{Smoke Stylization}
\Fig{tnst_lnst} shows a direct comparison of LNST and TNST applied to the smoke jet dataset of Kim et al. \shortcite{Kim2019}. While the resulting structures inherently depend on the underlying representation, they naturally differ and cannot be directly compared with each other. It can be observed, however, that the Lagrangian stylization may lead to more pronounced structures, well visible in the semantic transfer \emph{net} and the style transfer \emph{blue strokes}, and that boundaries are smoother, noticeable in the \emph{Seated Nude} example.

%
\begin{figure*}[h!]
\newcommand*{\mywidth}{0.158}
 \newcommand*{\triml}{350.0}
 \newcommand*{\trimr}{280.0}
 \newcommand*{\trimb}{0.0}
 \newcommand*{\trimt}{40}
 \centering
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/net_gt_105.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/net_new_105.jpg}
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/TNST_LNST/net_input_44.jpg}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/stroke_new_105.jpg}
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/TNST_LNST/stroke}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/nude_new_105.jpg}
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/TNST_LNST/nude}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/fire_new_105.jpg}
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/TNST_LNST/fire}
    \\
    \hspace{\mywidth\textwidth} 
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/net_old_105.jpg}
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/stroke_old_105.jpg}
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/nude_old_105.jpg}
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/TNST_LNST/fire_old_105.jpg}
    %\\
    % \vspace{1pt}
    %
    \caption{Semantic transfer applied to the smokejet simulation of \cite{Kim2019} (leftmost column). Stylized results are shown for our \add{LNST} (top) and TNST (bottom) for semantic feature transfer \emph{net} (second column) and input images \emph{blue strokes}, \emph{Seated Nude}, and \emph{fire} (last three columns)\protect\footnotemark.}
\label{fig:tnst_lnst}
\end{figure*}
%

\paragraph{Multi-fluid Stylization}
Stylization of multiple fluids is naturally enabled by stylizing different sets of particles with different input images. \Fig{multifluid} shows a simulation of two smoke jets colliding, where the left one is stylized with the semantic feature \emph{net} and the right one with the style transfer of the input image \emph{spirals}. Transferred structures are retained per fluid type even if the flow undergoes complex mixing effects. 

\begin{figure*}[th!]
\newcommand*{\mywidth}{0.26}
\newcommand*{\triml}{200.0}
 \newcommand*{\trimr}{230.0}
 \newcommand*{\trimb}{40.0}
 \newcommand*{\trimt}{60.0}
  \centering
\includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip,width=\mywidth\textwidth]{fig/results/multifluid/net_spi_0040.jpg}
\hspace{-53px}\includegraphics[width=0.1\linewidth]{fig/teaser/spirals_net.jpg}
\includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip,width=\mywidth\textwidth]{fig/results/multifluid/net_spi_0070.jpg}
\includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip,width=\mywidth\textwidth]{fig/results/multifluid/net_spi_0100.jpg}
  \caption{Two colliding smoke jets, which are stylized individually with the semantic feature \emph{net} and input image \emph{spirals}. The Lagrangian representation enables coherent stylization of multiple fluids even if the flow undergoes complex mixing.}
\label{fig:multifluid}
\end{figure*}
%

\paragraph{Stylization of Liquids}
We use a simple differentiable renderer for stylization of liquids. Unlike smoke renderer, which integrates media radiance scattered in the medium, we compute the amount of diffused light, \ie absorbed light except transmitted by its liquid volume~\cite{ihmsen2012unified}, which is given by 
%
\begin{equation}
\begin{split}
\tau(\vec{x}, \vec{r}) = e^{-\gamma \int_{\vec{0}}^{\vec{x}} d(\vec{r}) \; dr} \\
I_{ij} = 1 - \tau(\vec{r}_{max}, \vec{r}).
\label{eq:liquidRenderingEquation}
\end{split}
\end{equation}
%
\Fig{chocolate} shows the results of a stylized SPH simulation computed with \emph{SPlisHSPlasH}~\cite{splishsplash}. We applied the patterns \emph{spiral} and \emph{diagonal} to a thin sheet simulation.
%  
\begin{figure}[h!]
\newcommand*{\mywidth}{0.14}
 \newcommand*{\triml}{320.0}
 \newcommand*{\trimr}{300.0}
 \newcommand*{\trimb}{0.0}
 \newcommand*{\trimt}{50}
 \centering
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/liquids/gt_buckling_87.jpg} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/liquids/buckling_spiral_87.jpg} 
    \hspace{-26.6px}\includegraphics[width=0.1\linewidth]{fig/results/liquids/pattern1}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/liquids/buckling_square_87.jpg} 
    \hspace{-26.6px}\includegraphics[width=0.1\linewidth]{fig/results/liquids/square.jpg}
    %
    \caption{
 Thin sheet SPH simulation computed with \emph{SPlisHSPlasH}~\cite{splishsplash} stylized with the patterns \emph{spiral} and \emph{diagonal}.    
    }
%}
\label{fig:chocolate}
\end{figure}
%
\footnotetext{Image sources: \url{http://storage.googleapis.com/deepdream/visualz/tensorflow_inception/index.html},~
\url{https://github.com/byungsook/neural-flow-style}}

\paragraph{Color Transfer}
We transfer color information from input images to flow fields by storing a color value per particle and optimizing it by \Eq{LNSTloss}. This can be applied to any grid-based or particle-based smoke or liquid simulation. In \Fig{color} we applied the color stylization to a 2D dam break simulation using different example images, and in \Fig{colormix} to two liquids with distinct types (and hence color).
The accompanying videos show that local color structures change very smoothly over time, which is attributed to the improved time-coherency of the Lagrangian stylization. This is especially well visible in \Fig{colorSmoke}, where two subsequent frames are shown for TNST and LNST. In this example, we have transferred the style \emph{blue stroke} to a smoke scene. The close-up views reveal discontinuities for TNST, while LNST shows smooth transitions for color structures.

%
\begin{figure*}[t!]
\newcommand*{\mywidth}{0.31}
 \newcommand*{\triml}{0.0}
 \newcommand*{\trimr}{0.0}
 \newcommand*{\trimb}{0.0}
 \newcommand*{\trimt}{200}
 \centering
    \includegraphics[trim=\triml px \trimb px 0px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/wave_025} 
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/color/wave}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/wave_121} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/wave_199} 
    %
    \\
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/cokeffe_025} 
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/color/cokeffe}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/cokeffe_121} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/cokeffe_199} 
    \\
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/starry_025} 
    \hspace{-27.7px}\includegraphics[width=0.05\linewidth]{fig/results/color/starry}
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/starry_121} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/starry_199} 
    %\\
    % \vspace{1pt}
    %
    \caption{Lagrangian color stylization applied to a 2D particle-based liquid simulation using the input images \emph{Kanagawa Wave}, \emph{Red Canna} and \emph{Starry Night}.}
%}
\label{fig:color}
\end{figure*}
%
%
\begin{figure*}[t!]
\newcommand*{\mywidth}{0.31}
 \newcommand*{\triml}{0.0}
 \newcommand*{\trimr}{0.0}
 \newcommand*{\trimb}{0.0}
 \newcommand*{\trimt}{150}
 \centering
    \includegraphics[trim=\triml px \trimb px 0px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/ddam020} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/ddam040} 
    %
    \includegraphics[trim=\triml px \trimb px \trimr px \trimt px, clip, width=\mywidth\textwidth]{fig/results/color/ddam090} 
    %
    \caption{Lagrangian color stylization applied to a \emph{mixed} 2D particle-based liquid simulation using the input images \emph{Kanagawa Wave} and \emph{fire}.}
%}
\label{fig:colormix}
\end{figure*}
%

\section{Discussion and Conclusion}

We have presented a Lagrangian approach for neural flow stylization and have demonstrated benefits with respect to quality (improved temporal coherence), performance (stylization per frame in less than a minute), and art-directability (multi-fluid stylization, color transfer, liquid stylization). A key property of our approach is that it is not restricted to any particular fluid solver type (i.e., grids, particles, hybrid solvers). To enable this, we have introduced a strategy for grid-to-particle transfer (and vice versa) to efficiently update attributes and gradients, and a re-simulation that can be effectively applied to grid and particle fluid representations. This generality of our method facilitates seamless integration of neural style transfer into existing content production workflows. 

A current limitation of the method is that we use a simple differentiable renderer for liquids. While this works well for some scenarios, a dedicated differentiable renderer for liquids would improve the resulting quality and especially also support a wider range of liquid simulation setups. Similar to the smoke renderer, such a liquid renderer must be differentiable as gradients are back-propagated in the optimization. It must also be efficient as the renderer is used in each step of the optimization. Although the complexity of the renderer has a direct influence on the quality of the results, we suspect that, analogously to our smoke renderer, a lightweight renderer that can recover the core flow structures is sufficient for stylizing liquids.

We have shown that LNST enables novel effects and a high degree of art-directability, which renders flow stylization more practical in prodcution workflows. However, we have not tested the method on large-scale simulations that are typically used in such settings. While our method can handle up to 2 million particles, larger scenes are restricted by the available memory. Moreover, in practical settings the scene complexity is higher, which potentially poses challenges with respect to artist control of the stylization. 

By reducing the computation time for stylizing an entire simulation from one day with TNST to a single hour with LNST renders the method much more practical for digital artists. However, for testing different input structures, a real-time method would be desirable. Recent concepts presented on neural image stylization might be mapped to 3D simulations to further improve efficiency.  


